Robotic Agentic Platform for Intelligent Electric Vehicle Disassembly

Electric vehicles (EV) create an urgent need for scalable battery recycling, yet disassembly of EV battery packs remains largely manual due to high design variability. We present our Robotic Agentic Platform for Intelligent Disassembly (RAPID), designed to investigate perception-driven manipulation, flexible automation, and AI-assisted robot programming in realistic recycling scenarios. The system integrates a gantry-mounted industrial manipulator, RGB-D perception, and an automated nut-running tool for fastener removal on a full-scale EV battery pack. An open-vocabulary object detection pipeline achieves 0.9757 mAP50, enabling reliable identification of screws, nuts, busbars, and other components. We experimentally evaluate (n=204) three one-shot fastener removal strategies: taught-in poses (97% success rate, 24 min duration), one-shot vision execution (57%, 29 min), and visual servoing (83%, 36 min), comparing success rate and disassembly time for the battery's top cover fasteners. To support flexible interaction, we introduce agentic AI specifications for robotic disassembly tasks, allowing LLM agents to translate high-level instructions into robot actions through structured tool interfaces and ROS services. We evaluate SmolAgents with GPT-4o-mini and Qwen 3.5 9B/4B on edge hardware. Tool-based interfaces achieve 100% task completion, while automatic ROS service discovery shows 43.3% failure rates, highlighting the need for structured robot APIs for reliable LLM-driven control. This open-source platform enables systematic investigation of human-robot collaboration, agentic robot programming, and increasingly autonomous disassembly workflows, providing a practical foundation for research toward scalable robotic battery recycling.

==> tab_cost_ablation.tex <==
\begin{table}[t]
\caption{Cost function ablation results (avg.\ over successful plans).
\textbf{Bold} = best, \underline{underline} = second best.}
\label{tab:cost-ablation}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l ccccc}
\toprule
Config. & SR (\%)$\uparrow$ & Plan (s)$\downarrow$ & Exec (s)$\downarrow$ & Path (m)$\downarrow$ & Manip.$\uparrow$ \\
\midrule
Base & \textbf{99.6} & 0.96 & 6.24 & 2.40 & 0.481 \\
\midrule
Area & 99.0 & 0.53 & 6.28 & 2.52 & 0.421 \\
Joint & 98.3 & 0.56 & 4.53 & \underline{1.64} & 0.489 \\
Prox & 99.3 & 0.38 & 4.24 & 1.87 & \textbf{0.700} \\
\midrule
~Area & \underline{99.4} & 0.48 & 4.33 & 1.78 & \underline{0.699} \\
~Joint & 99.1 & \underline{0.27} & 4.26 & 2.01 & 0.642 \\
~Prox & 97.9 & 0.27 & \textbf{3.98} & \textbf{1.52} & 0.424 \\
Equal & 99.3 & \textbf{0.22} & \underline{4.10} & 1.70 & 0.628 \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tab_rrt_corridor.tex <==
\begin{table}[!t]
\caption{Unconstrained RRT vs.\ corridor-constrained planning over 1\,000 random
goal poses. RRT uses the no-area cost configuration selected in
Section~\ref{sec:cost}. Averages are over successful plans only.
\textbf{Bold} = best per column.}
\label{tab:rrt-corridor}
\centering
\begin{tabular}{l cccc}
\toprule
Strategy & SR (\%)$\uparrow$ & Plan (s)$\downarrow$ & Path (m)$\downarrow$ & Exec (s)$\downarrow$ \\
\midrule
Pure RRT  & \textbf{99.4} & \textbf{0.51} & 1.78          & \textbf{4.36} \\
Corridor  & 93.4          & 47.4          & \textbf{1.26} & 7.12 \\
\bottomrule
\end{tabular}
\end{table}

